Can Multimodal Large Language Models Truly Perform Multimodal In-Context Learning?

Large Language Models (LLMs) with in-context learning (ICL) ability can quickly adapt to a specific context given a few demonstrations (demos). Recently, Multimodal Large Language Models (MLLMs) built upon LLMs have also shown multimodal ICL ability, i.e., responding to queries given a few multimodal demos, including images, queries, and answers. While ICL has been extensively studied on LLMs, its research on MLLMs remains limited. One essential question is whether these MLLMs can truly conduct multimodal ICL, or if only the textual modality is necessary. We investigate this question by examining two primary factors that influence ICL: 1) Demo content, i.e., understanding the influences of demo content in different modalities. 2) Demo selection strategy, i.e., how to select better multimodal demos for improved performance. Experiments revealed that multimodal ICL is predominantly driven by the textual content whereas the visual information in the demos has little influence. Interestingly, visual content is still necessary and useful for selecting demos to increase performance. Motivated by our analysis, we propose a simple yet effective approach, termed Mixed Modality In-Context Example Selection (MMICES), which considers both visual and language modalities when selecting demos. Extensive experiments are conducted to support our findings and verify the improvement brought by our method. Code is available at \url{https://chenxshuo.github.io/m-icl/}.

==> sections/3-2-new-exps.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[clip, width=0.95\columnwidth]{figures/understand-attn-OF-9b.pdf}\vspace{-0.2cm}
\caption{The left figure shows the cosine similarity between hidden states in the standard setting and removing images in the demos (blue bars). Grey bars are cosine similarity between standard setting and removing query images. The right figure shows the similarity of the corresponding attention weights in the last decoder layer. Omitting demonstration visual embeddings leads to similar hidden states, but excluding query images increases their dissimilarity.
}\vspace{-0.3cm}
\label{fig:OF-cosine}\vspace{-0.3cm}
\end{figure}


\subsection{Further Investigation to Understand the Content Influence}
\label{sec:new-exps}
% 1. performance from models w/ auto regressive structure 

Previous subsections highlight the dominant role of textual information in ICL for MLLMs, yet leave several questions unanswered: 
1) Why do the images in demos barely affect the ICL performance, and why can the text dominate the ICL ability for the MLLMs? 
2) Do these results also apply to MLLMs using other model architectures? 
3) Do these results depend on the evaluation task? 

For the first question, existing literature~\cite{li2023otter, zhao2023mmicl, li2023mimic, doveh2024towards} shows that the pre-training datasets cannot provide sophisticated context information and may limit the ICL ability of the trained MLLMs. 
To further investigate the reasons, this work studies the model structures, \ie, masked cross attention, and analyzes the influence of multimodal demos. Specifically, we compare the self-attention weights and self-attention outputs of the language decoder block in the standard setting with two scenarios, \ie, with and without providing visual information in demos. 
If the combination of masked cross-attention across modalities and the self-attention on text tokens maintains the dependency on previous images, excluding visual information from previous demonstration images will lead to different attention behaviors, \eg, different attention weights and hidden states. Otherwise, if the weights and hidden states remain almost the same after removing visual information in the demos, the model does not attend much to previous demonstration images. 
Specifically, we compute the cosine similarity on the last row of hidden states and attention weights in the last decoder layer for each generation forward and then average the results over the whole dataset. 
To remove the visual information in the demos, we mask the visual embeddings of the demo images, by setting the weights to $0$ and keeping the query image embedding.
% To remove the visual information in the demos, we mask the visual embeddings of the demo images, such as $\mathbf{I_1}$ and $\mathbf{I_2}$, by setting the weights to $0$ and keeping the query image embedding $\mathbf{I_q}$. 
\cref{fig:OF-cosine} presents the results. Removing demonstration visual embeddings leads to around $90\%$ similar hidden states whereas excluding query images makes the hidden states much more dissimilar. 
These differences in similarity highlight the insignificance of demo images for existing MLLMs in ICL. 

% 
To answer the second question, we have conducted additional experiments on Qwen-VL-Chat~\cite{bai2023qwen}, and the results are presented in \TODO{TOADD}.

The third question points out that the observation in previous sections could be caused by the VL tasks used for evaluation. 
For example, captioning the query image can depend on the query image content and the desired output format indicated by the text in the demos, whereas the usefulness of demo images is somewhat hard to measure. 
To further examine the multimodal ICL ability, we adopt a new task Operator Induction (OI)~\cite{zong2024vl}, which explicitly requires the focus on the demo images for the correct answer. 
In OI, the models need to generate responses for a query image \eg, $2\ ?\ 7 =$, given context images showing \eg, $2\ ?\ 4 = 6$. 
The models must induce the correct operator from the demo images and use the operator to calculate the correct answer for the query, \eg, $9$ as the induced operator should be $+$, for the previous example. 
A concrete example is shown in~\cref{fig:OI}. 
Besides directly hiding the demo images, a new setting is designed, in which the demo image content is directly added to the demo text, \ie, the optical character recognition (OCR) results of demo images, as shown in~\cref{fig:OI-d}. 
In total, there are 4 different settings 


==> sections/old-1-introduction.tex <==
% In-context learning (ICL) on large language models (LLMs) has shown surprisingly good performance in generating responses to queries by only observing a few demonstrations without any parameter updates. 
% Recent vision-language models (VLMs) exhibits in-context learning (ICL) capability where the model can respond to queries by conditioning on a series of multimodal demonstrations including images, queries, and answers. 
% Although ICL has been widely studied on large language models, related research on VLMs is still rare. Besides, the additional incorporated visual information in the demonstrations raises new research questions, \eg, which part of the information in the demonstration is more important? how to better select multimodal demonstrations for better ICL performance? 
% This work first explores the importance of visual and language information and reveals that the textual part is essential for VLMs to perform ICL. Removing images from the demonstrations barely decreases the ICL performance. 
% We then examine the way to condition pre-trained LLMs on visual representations in VLMs. We find out that images in the demonstrations are not as important as images in the query. Visualization of the model weights further underpins such understanding. 
% Based on our analysis, we design a simple yet effective method, namely Visual-then-Language In-Context Example Selection (VLICES), which first filters candidates via visual similarity and then selects demonstrations based on language similarity.  
% Extensive qualitative and quantitative experiments are conducted to support our findings, understanding, and further improvement of the ICL performance of VLMs. 


%we examine the methodology of conditioning pre-trained LLMs on visual representations within VLMs. It is revealed that images included in the demonstrations are not as influential as textual data. Further evidence supporting this understanding is provided through the visualization of the model weights. 

% old abstract 
%ICL on VLMs is good
Vision-language models (VLMs) enhanced with large language models (LLMs) have demonstrated remarkably powerful few-shot in-context learning (ICL) capabilities. In this process, the VLMs are adapted to a new task by observing only a few context demonstrations, without the need for any gradient updates.
% how to find better support examples is not clear
However, there is still a lack of understanding of ICL and the exploration of finding better supporting examples. Most of the existing work has only focused on investigating ICL on LLMs. However, ICL on VLMs is quite different due to the diverse modality and flexible context, and therefore requires further investigation.
% what we find
This study represents an initial exploration of the image captioning language (ICL) ability of VLMs. Our findings indicate that the language information within the context significantly influences ICL performance. Furthermore, we examine the attention and hidden states within the model, uncovering that VLMs assign lower attention to input images.
Based on our analysis, we have developed a simple yet effective strategy to effectively select demonstrations for ICL on VLMs. named Visual-then-Language In-Context Example Selection (VLICES), which demonstrates significant performance improvements compared to existing methods.
Extensive qualitative and quantitative experiments are conducted to support our findings, understanding, and further improvement of the ICL performance of VLMs. 


\section{Introduction}
% Structure 
% ICL on NLP and VLs are useful and powerful， but understanding is lacking 
% Many works have tried to understand the mechanism of ICL on NLP tasks. 
% VL tasks are different and it is hard to follow the ICL-NLP field findings directly. 
% We take the first step to understand and improve ICL ability on VL tasks 
% We find that ... 
% We propose .. method to enhance the ICL ability across various VL tasks ...


%%Jindong's Sotry
% START ---------------

% ICL on LLM has received great attention from community, 一句话解释question and answer demo，优点improve model performance without requiring parameter updates。最近的基于 LLM的 VLM 也展示出了 ICL的能力，一句话解释 VLM上的ICL。while LLM ICL intensively studied, ICL on VLM poorly understood. Different from ICL on LLM, ICL on VLM 包含了更多的visual information。It is not clear which of visual info and textual info is more important to the ICL performance and how to choose effective demo for ICL on VLM.


% --findings-- In this work, we explore the questions, we first conduct experiments where 我们如何ablate的 across various tasks and model variants，we found that textual information is critical for ICL, ignoring the visual info hardly degrades ICL performance.

% --understanding-- To understand the observation, we first analyze the Masked cross attention, a popular way to integrate visual information. Our analysis shows demo 中的图像不重要，query 中的图像很关键。 we further visualize the information flow, The visualization further verify that visual information in demos has only slight impact on model output, while the query images is directly related to model outputs

% --improvements-- based on our analysis above, we propose a simple, yet effective approach to select effective demos for ICL on VLM. Concretely, 两句话解释我们的方法，两句话解释这么做为什么好，一句话说extensive experiment verify our proposed method across models and datasets

% Summary of contributions
% \item \textbf{Finding}: We study ICL on VLM. Through extensive experiments, we discovered that language information is more crucial than visual information in the demonstrations. 忽略images 在ICL的demo 中几乎不降低 ICL performance

% \item \textbf{Understanding}: we analysis the core design to integrate visual information, we revealed that， we further visualize the information flow/attention to further support our analysis

% \item \textbf{Improvement}: Motivated by our findings and understanding, we propose a simple, yet effective VLICES to enhance the in-context learning performance of pre-trained vision-language models. 

% END ---------------

The in-context learning (ICL) ability of large language models (LLMs) has received great attention 








%%%%%%%%%%%%%%%%%%%%%%%% OLD Version 

Vision-language models (VLMs) pre-trained on massive multimodal datasets have made significant progress~\cite{radford2021learning, cho2021vlt5, tsimpoukelli2021multimodal, li2023blip, huang2023language, driess2023palm, liu2023visual, alayrac2022flamingo,peng2023kosmos}, demonstrating surprisingly powerful in-context learning ability~\cite{alayrac2022flamingo, laurenccon2023obelisc, tsimpoukelli2021multimodal, awadalla2023openflamingo, zhao2023mmicl, peng2023kosmos}.
In-context learning ability is first observed in large language models (LLMs)~\cite{brown2020language, touvron2023llama, hoffmann2022an, chowdhery2022palm, liang2022holistic} where the model learns to do a new task simply by conditioning on context prompts with a few input-output pairs. Benefiting from these powerful LLMs and web-scale vision-language datasets, many recent VLMs also possess such capability~\cite{tsimpoukelli2021multimodal, alayrac2022flamingo, zhao2023mmicl, peng2023kosmos}. 
Such ICL capability spurs a new paradigm of using pre-trained VLMs~\cite{bommasani2021opportunities, dong2022survey} and makes it much easier to incorporate human knowledge into pre-trained models via demonstrations and templates~\cite{liu-etal-2022-makes, wu2022self, wei2022chain} and reduces the cost of adapting the model to new tasks~\cite{sun2022black, alayrac2022flamingo, zhao2023mmicl}. 
%Besides, in-context learning is similar to the learning process of human beings by learning from analogy~\cite{winston1980learning} and provides an interpretable interface to communicate with pre-trained models~\cite{brown2020language}.  

Although ICL has proven to be effective, there is still a lack of understanding regarding its ability, and most of the existing research has only focused on investigating the mechanism on LLMs~\cite{min-etal-2022-rethinking, yoo-etal-2022-ground, wei2023larger, lu-etal-2022-fantastically, liu-etal-2022-makes, an-etal-2023-context, olsson2022context, bansal2022rethinking, akyrek2023what, von2023transformers, dai2023can, li2023closeness}. 
% Some unintuitive conclusions have been dawn on LLMs, such as .... 
However, the ability of vision-language models (VLMs) to perform in-context learning is quite different. This is because: 1) VLMs are pre-trained on interleaved image-text datasets, which makes the task and the model more complicated compared to pure language datasets. 2) The context prompts in VLMs can include extra visual information and offer more flexibility. 3) Vision-language tasks in VLMs are solved through text generation, unlike the closed-word classification studied in ICL on language-only models (LLMs). Therefore, it is not advisable to directly apply the findings from LLMs to VLMs.
Besides, current studies of ICL on VLMs are mainly about proposing larger multimodal datasets~\cite{laurenccon2023obelisc} and designing models with better ICL ability~\cite{tsimpoukelli2021multimodal, alayrac2022flamingo, zhao2023mmicl}.
%and directly improving the ICL performance~\cite{alayrac2022flamingo, awadalla2023openflamingo} such as using RICES~\cite{alayrac2022flamingo, awadalla2023openflamingo}, \ie, selecting demonstrations based on image similarity. 
Some work~\cite{yang2022empirical, alayrac2022flamingo, awadalla2023openflamingo} shows that Retrieval-based In-context Example Selection (RICES) leads to better ICL performances, \ie, selecting demonstrations based on image similarity. 
However, there is no research specifically addressing the understanding of the ICL ability of VLMs. This lack of research has left several crucial questions unanswered: 
\begin{itemize}
\item Do VLMs rely more on language information or visual information in the context demonstrations? 
\item Which type of information is most important for the ICL ability of VLMs? Is it images, questions, or labels? 
\item What is the reason behind the improved ICL performances achieved through the use of RICES?
\end{itemize}
To this end, this study examines the in-context learning capability of VLMs, in order to address the aforementioned research questions. Specifically, we initially performed extensive empirical experiments on VLMs of various sizes, ranging from 3B to 9B. These experiments are conducted on four vision-language task datasets: VQAv2~\cite{antol2015vqa}, OK-VQA~\cite{okvqa}, GQA~\cite{hudson2019gqa}, and MSCOCO Caption~\cite{chen2015microsoft}. We observe that language information plays a vital role in the ICL settings and VLMs can achieve comparable ICL performances without the aid of visual information in the context examples. Among the provided language information, proper exposure to the correct label space is the most significant factor for achieving satisfactory ICL performance.
Then we delve into the attention and hidden states inside the model to understand model behaviors. Experiments demonstrate that the masked cross-attention mechanism weakens the dependency of VLMs on the visual information in the demonstrations. The retrieved similar images from RICES do not directly boost the ICL performance, instead, the performance boost comes from the accompanying language information associated with the demonstration images.

Last but not least, we have developed a simple yet effective ICL strategy called Visual-then-Language In-Context Example Selection (VLICES), based on our observations and findings. VLICES surpasses existing example selection methods in various settings. It utilizes a two-stage selection mechanism that initially chooses candidates based on image similarity and then further ranks them based on text similarity.
VLICES outperforms RICES and random selection by a significant margin. It shows an improvement of up to $8.8\%$ on VQAv2, $5.1\%$ on OK-VQA, $10.3\%$ on GQA, and $10.9\%$ on MSCOCO.



% a figure showing ICL ability and some examples showing the uselessness of images 
\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{figures/alg-diagram.pdf}
  \caption{\label{fig:alg-diagram} Visual-then-Language In-Context Example Selection (VLICES) in VQA. In the first stage, VLICES selects candidate examples based on visual similarity. Then language similarity is used in the second stage to further rank and select context examples. }
% \caption{\label{fig:ICL-examples} VLMs can do in-context learning (first row) even with mismatched images (bottom row). Given a few demonstrations (\eg, 2 image-text pairs in this figure), the model can adapt to a task quickly such as the VQA task. }
\end{figure}

% Add a figure to show how our method works. TODO 


To summarize, our main contributions are as follows:
\begin{itemize}
    \item \textbf{Finding}: Through extensive experiments, we discovered that language information is more crucial than visual information in the demonstrations. Additionally, it is necessary to ensure correct label space exposure. Surprisingly, even blank images and out-of-distribution images can yield similar results.
    \item \textbf{Understanding}: We found that the models prioritize the language input over the visual information provided in the context demonstrations. As a result, complex visual information may not be fully understood and utilized in the ICL setting.
    \item \textbf{Improvement}: Motivated by our findings and understanding, we propose VLICES to enhance the in-context learning performance of pre-trained vision-language models. VLICES outperforms existing methods by a significant margin across various datasets.
\end{itemize}

% method name Cross Modality Selection 

==> sections/old-2-related-work.tex <==
\section{Related Work}
\vspace{0.1mm}
\noindent\textbf{In-context Learning on Vision-Language Models.}Frozen~\cite{tsimpoukelli2021multimodal} is the first attempt for ICL in multimodality by leveraging a frozen GPT-like LM as the language backbone and mapping visual features to the language embedding space. Flamingo~\cite{alayrac2022flamingo} is the first state-of-the-art in-context learning VLM which also supports flexibly interleaved image-text input. Besides, Otter~\cite{li2023otter} and MMICL~\cite{zhao2023mmicl} further augment the in-context learning ability by training in datasets with more complex contexts.
Apart from proposing pre-trained VLMs with in-context learning ability, some have explored better in-context configurations for image captioning~\cite{yang2023exploring}. Some work aims to alleviate the dependency on large-scale pre-training. For instance, SINC~\cite{chen2023sinc} enables in-context learning without relying on the intrinsic in-context ability of large language models. \citeauthor{monajatipoor2023metavl} studied how to transfer in-context learning ability from large language models to vision-language models without relying on extensive scalability. Apart from these, ICL is also used as a tool to reduce the flaws of large multimodal models such as hallucination and abstention~\cite{shukor2023beyond}. 
Different from all of prior work, our study focuses on the understanding of the in-context learning ability of vision-language models. 
%Compared to in-context learning studies on large language models, there is less research specifically dedicated to in-context learning on vision-language models. 


\vspace{0.1mm}
\noindent\textbf{Understanding In-Context Learning.} 
Large language models have demonstrated the surprising and competitive in-context few-shot learning ability~\citep{brown2020language, touvron2023llama, hoffmann2022an, chowdhery2022palm, liang2022holistic}, \ie, adapting to a new task conditioned on a few in-context demonstrations without any gradient update. 
Despite its effectiveness and efficiency, the mechanism of in-context learning ability is not yet fully understood. \citeauthor{min-etal-2022-rethinking} examined the role of in-context demonstrations from four aspects, \ie, label space exposure, the distribution of demonstration input, the format of input-label pairing, and the input-label mapping of demonstrations. 
\citeauthor{min-etal-2022-rethinking} concluded that the input-label mapping is not essential as expected whereas the other three factors have much more influence on the in-context learning performance. 
However, \citeauthor{yoo-etal-2022-ground} found that correct demonstration labels actually impact the ICL performance in certain specific scenarios. 
\citeauthor{wei2023larger} indicated that different model scales could lead to different interactions between semantic priors learned in pre-training and input-label mappings given in demonstrations. 
Moreover, \citeauthor{lu-etal-2022-fantastically} studied the problem of order sensitivity. Some works also investigated the relationship between the ICL performance and demonstration similarity~\citep{liu-etal-2022-makes}, diversity~\citep{an-etal-2023-context}, and complexity~\citep{an-etal-2023-context}. 
Besides, There are also works studying ICL from the distribution of training data~\cite{chan2022data, han-etal-2023-understanding}, from the transformer architecture~\cite{olsson2022context, bansal2022rethinking}, connecting ICL with gradient descent~\cite{akyrek2023what, von2023transformers, dai2023can, li2023closeness}, and investigating the learning algorithm~\cite{garg2022can, pmlr-v202-li23l, pan-etal-2023-context, hahn2023theory, si-etal-2023-measuring}. 
All of these work focuses on ICL of large language models and most of them only study basic tasks such as text classification~\cite{min-etal-2022-rethinking, yoo-etal-2022-ground, wei2023larger, lu-etal-2022-fantastically}. However, VLMs are different from LLMs due to the inclusion of visual information, which allows for more flexible and diverse tasks. Understanding the ICL ability of VLMs requires further investigation. To our knowledge, there is currently no research that specifically focuses on understanding the ICL ability of VLMs.
%Our task, \ie, ICL ability of vision-language models, is quite different because 1) models are pre-trained on interleaved image-text datasets rather than pure language datasets; 2) the context prompts include images and are more flexible; and 3) vision-language tasks are solved via text generation rather than closed-word classification. Hence, 


\vspace{0.1mm}
\noindent\textbf{Vision-Language Models.} % emphasize the models with ICL ability  
Pre-trained vision-language models~\cite{li2020unimo, radford2021learning, li2019visualbert, su2019vl, cho2021vlt5, tan2019lxmert, alayrac2022flamingo, tsimpoukelli2021multimodal} have demonstrated outstanding performance on various VL tasks. 
Some use contrastive learning to align visual features with language representations and achieve surprising zero-shot performance \cite{li2020unimo, radford2021learning}. However, contrastive learning-based methods are limited to close-ended tasks such as image classification and are inflexible. 
Another line of work follows BERT's \cite{devlin2018bert} pretrain-then-finetune paradigm \cite{li2019visualbert, su2019vl, cho2021vlt5, tan2019lxmert}. They treat object features extracted using pre-trained object detectors \cite{girshick2015fast} as visual words sent to language models \cite{devlin2018bert}. However, these pre-trained VL models require extra fine-tuning to better adapt to a specific downstream application. More recently, some VLMs~\cite{li2023blip, huang2023language, driess2023palm, liu2023visual} are built on top of powerful pre-trained large language models and freeze the LM weights to prevent catastrophic forgetting and better utilize the LM's autoregressive text generation capacity. However, they either only support the fixed format of image-text input, \eg, single images, rather than flexible arbitrarily interleaved image-text content, or do not possess in-context learning ability.
Flamingo~\cite{alayrac2022flamingo} is the first VLM that can both ingest arbitrarily interleaved image-text input and demonstrate powerful few-shot in-context learning ability. Despite being closed-source, several public reproductions of Flamingo are available~\cite{laurenccon2023obelisc, alayrac2022flamingo} with comparable performance, which make further research possible. In this study, we mainly focus on two public competitive reproductions, \ie OpenFlamingo~\cite{awadalla2023openflamingo} and IDEFICS~\cite{laurenccon2023obelisc}, which are on par with Flamingo on various multimodal benchmarks~\cite{laurenccon2023obelisc, alayrac2022flamingo}. They differ in the size and selection of training data, where OpenFlamigo is trained on LAION-2B~\cite{schuhmann2022laion} and Multimodal C4~\cite{zhu2023multimodal}, and IDEFICS is trained on OBELICS~\cite{laurenccon2023obelisc}.




==> sections/old-3-2-attention-zhen.tex <==
\section{Understanding Multimodal Information Flow inside Model}
\label{sec:attention}

The empirical examination outlined in Sec.~\ref{sec:understanding} underscores the dominant role of textual information in ICL for VLMs, yet leaves several questions unresolved: 1) Why do the images in context demonstrations barely affect the ICL performance? 2) Why is the query image still useful? To fully investigate the underlying reasons, this section delves into the model details to analyze the influence of both visual and language information in the context demonstrations. 

% on the flamingo's mechanism and our guess
VLMs with ICL ability (\eg, Flamingo) can handle interleaved text and visual sequences, making in-context few-shot learning possible~\cite{alayrac2022flamingo}. 
An illustration is presented in Fig.~\ref{fig:OF-attention}, with two demonstrations and a query, each of which contains an image and corresponding text such as $I_1$ and $T_1$ in the first demonstration. 
The masked cross-attention layer enables the language models to incorporate visual information for the next-token prediction. This layer also limits which visual tokens the model sees at each text token. 
Specifically, at a given text token, the model only attends to the visual tokens of the last preceding image, rather than to all previous images in the interleaved sequence. 
For example, text embedding $T_q$ can only attend to the image $I_q$ in the masked cross-attention layer.
Therefore, demonstration images $I_1$ and $I_2$ cannot directly pass their visual information to the query text embedding $T_q$, as $T_q$ is limited to interacting with the query image $I_q$ in the masked cross-attention layer. 
Only in the subsequent self-attention layer can $T_q$ indirectly access the information from $I_1$ /$I_2$ through the demonstration text embeddings $T_1$ and $T_2$, which have already processed the visual information from these images in the masked cross-attention layer. 
We argue that the masked cross-attention mechanism with such per-image attention masking~\cite{alayrac2022flamingo} complicates the realization of text tokens' dependency on all previous images. 
In other words, relying solely on the self-attention layer for transferring visual information to text tokens is difficult.
Thus, in the ICL settings, we see the generated output tokens primarily focus on the latest image, i.e., the query image. However, it largely disregards the visual information of the previous demonstration images.

==> sections/old-3-understanding.tex <==
\section{Understanding In-context Learning Ability on Vision-language models}
\label{sec:understanding}
This section examines the behavior of the VLMs in various ICL settings. Section \ref{sec:understanding:role_of_image} analyzes the impact of images in the demonstrations, while Section \ref{sec:understanding:label_space_exposure} investigates which information is most essential for good ICL performance. Additionally, Section \ref{sec:understanding:demo_input_dist} explores the influence of demonstration distribution and the format of input-label pairing.

\subsection{The role of images in ICL demos}
\label{sec:understanding:role_of_image}
\vspace{0.1mm}
\noindent\textbf{In-context Learning Settings.} % settings related to ICL 
In vision-language in-context learning, a query input $I_q$, \eg, an image \texttt{<image>} and a question/instruction $T_q$, coming after a context prompt $C$, is sent to a pre-trained vision-language model $M$. The context prompt $C$ consists of $N$ task demonstrations. Each demonstration includes demo $\texttt{<image>}_i$, demo instruction $T_i$, and demo response $R_i$. For instance, in VQA, $T$ is a question related to the input \texttt{<image>} and $o$ is generated as the answer to $T$. 
Then $M$ generates a response $o$ to the input $I$, \eg, the answer to $Q$, based on \texttt{<image>}. 
Specifically, the ICL can be written as follows~\cite{shukor2023beyond}:
\begin{equation}
\begin{gathered}
    o=M([C,I_q]),\\
    I_q=\langle\texttt{<image>},T_q \rangle, C=\{ \langle \texttt{<image>}_i, T_i, R_i \rangle \}_N.
\end{gathered}
\end{equation}
We follow traditional settings~\cite{awadalla2023openflamingo, laurenccon2023obelisc, alayrac2022flamingo} and set $N$ as $0, 4, 8, 16, 32$ in our experiments. 


% - draw 4 line graphs on 4 datasets (OF9B) 
Unlike ICL in LLMs, ICL in vision-language models incorporates visual information into the demonstration. This visual information can be in the form of images used for tasks like VQA or image captioning. In order to assess the impact of including correctly related images, also known as ground-truth images, in the demonstrations, we compare the following three settings.

\vspace{0.1mm}
\noindent\textbf{Demonstartions w/o images.}
In this setting, the visual information is removed from the demo context $C$ by deleting the $\texttt{<image>}_i$ in $C$. This results in the context $C$ with $N$ text-only instructions such as the questions in VQA or the captions in the task of image captioning, whereas the images for these questions and captions are removed from the demonstrations. The specific tokens indicating image positions in the demonstrations are also excluded, \eg, \texttt{<image>} in Flamingo~\cite{alayrac2022flamingo}. 

\vspace{0.1mm}
\noindent\textbf{Demonstartions w/ blank images.}
This setting keeps the images and image position tokens in the demonstrations but replaces the original images with blank images, \ie, all the pixel values are set to $255$. Although there are still images in the demonstrations, they do not provide any information. 

\vspace{0.1mm}
\noindent\textbf{Demonstartions w/ OOD images.}
Besides the two settings above, we replace the original images with random out-of-distribution (OOD) images, \eg, VQA-RAD~\cite{lau2018dataset} in our experiments.  VQA-RAD~\cite{lau2018dataset} is a manually constructed dataset where clinicians asked naturally occurring questions about radiology images and provided reference answers. The images in VQA-RAD are shown neither in model pre-training nor in downstream tasks used in our study and can be seen as a natural out-of-distribution dataset.


% demonstration with multiple objects? TODO 

% \begin{figure}[]
% \subfloat{%
%   \includegraphics[clip,width=\columnwidth]{figures/understand-images-OF-9b.pdf}%
% }

% \subfloat{%
%   \includegraphics[clip,width=\columnwidth]{figures/understand-images-IDEFICS-9b.pdf}%
% }
% \caption{\label{fig:understand-images}The performances of \texttt{OF-9B} and  \texttt{IDEFICS-9B} given different images demonstration settings.}
% \end{figure}


\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{figures/understand-images-OF-9b.pdf}
\caption{\label{fig:understand-images} The performances of \texttt{OF-9B} given different image demonstration settings. The horizontal lines are the zero-shot performance.}
\end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/understand-images-IDEFICS-9b.pdf}
% \caption{\label{fig:understand-images-idefics-9b} The performances of \texttt{IDEFICS-9B} given different image demonstration settings.}
% \end{figure}

The ICL performances given these different demonstration settings are presented in Fig.~\ref{fig:understand-images}, which also includes the performance without the query image. 
Compared with the ground-truth image setting and removing query image, both image removal and image replacement do not drop the ICL performances significantly. Some performances are even better than the ground-truth setting such as on the OK-VQA and GQA datasets. \texttt{IDEFICS-9B} shows a similar trend on VQA and visual reasoning tasks and for captioning. 
\textbf{Although there is a lack of useful visual information in the demonstrations, the performances remain relatively similar as long as the demonstrations contain valid instructions, \eg, correct question-label pairs for VQA and GQA.}
What we have observed here leads us to focus more on the language information in the context examples.

% \begin{figure}[]
% \subfloat{%
%   \includegraphics[clip,width=\columnwidth]{figures/understand-labels-OF-9b.pdf}%
% }

% \subfloat{%
%   \includegraphics[clip,width=\columnwidth]{figures/understand-labels-IDEFICS-9b.pdf}%
% }
% \caption{\label{fig:understand-labels}The performances of \texttt{OF-9B} and  \texttt{IDEFICS-9B} given different label demonstration settings.}
% \end{figure}

\begin{figure}
  \centering
  \includegraphics[width=1.0\linewidth]{figures/understand-labels-OF-9b.pdf}
\caption{\label{fig:understand-labels} The performances of \texttt{OF-9B} given different label demonstration settings.}
\end{figure}

\subsection{Label Space Exposure}
\label{sec:understanding:label_space_exposure}
% - 5 settings 
It has been shown that the exposure of correct label space is essential in ICL on LLMs~\cite{min-etal-2022-rethinking}, \ie, the space covered by the desired output such as the classification labels in text classification. In vision-language tasks, \eg, VQA and image captioning, the label space is broader than text classification on LLMs, especially when approached by text generation. Hence, the investigation of the influence of the label space on vision-language tasks is still necessary. Besides the default ground-truth setting, four additional scenarios are conducted, namely \textit{random strings as labels} (\ie, replaces the original labels with random ASCII strings), \textit{random words as labels} (\ie, replacing the original labels with random English words), and \textit{random other labels as labels} which contains \textit{random question labels as labels} and \textit{random labels from the same question as labels} for VQA and GQA tasks. 

The performance comparison is presented in Fig.~\ref{fig:understand-labels} where the above figure is from \texttt{OF-9B} and the below is \texttt{IDEFICS-9B}. In contrast to different image demonstrations, modifying the label space exposure has a more significant impact on the ICL performance. Replacing the labels with random strings and random words drops the ICL performances to nearly $0$ with only $4$ shots. For VQA and visual reasoning, random labels from the support dataset also decrease the performances and the negative impact is more severe with a larger number of examples. On the captioning task, random labels from the support dataset are image captions that are mismatched with the images in the demonstrations. Nevertheless, such a discrepancy results in a comparable performance on \texttt{OF-9B}. Random labels for the same question achieve comparable performances on VQA and visual reasoning, although the labels are incorrect w.r.t. the demonstration images. The labels from the same question are consistent with the question's meaning. For example, answers to questions like "Is it a cat?" should start with the form "Yes" or "No" and a random word as the answer would mislead the model. 

\begin{figure}[]
\subfloat{%
  \includegraphics[clip,width=\columnwidth]{figures/understand-input-OF-9b.pdf}%
}

% \subfloat{%
%   \includegraphics[clip,width=\columnwidth]{figures/understand-input-IDEFICS-9b.pdf}%
% }
\caption{\label{fig:understand-input}The performances of \texttt{OF-9B} given different input demonstration settings. The horizontal lines are the zero-shot performance.}
\end{figure}

\begin{figure}[]
\subfloat{%
  \includegraphics[clip,width=\columnwidth]{figures/understand-format-OF-9b.pdf}%
}

% \subfloat{%
%   \includegraphics[clip,width=\columnwidth]{figures/understand-format-IDEFICS-9b.pdf}%
% }
\caption{\label{fig:understand-format}The performances of \texttt{OF-9B} given different format of input-label pairing settings.}
\end{figure}

\subsection{Demonstration distribution and format}
\label{sec:understanding:demo_input_dist}
% - 4 settings 
In the demonstrations, some vision-language tasks also provide instructions such as the questions in VQA and GQA. The distribution of these input texts has been proven to provide learning signals in ICL on LLMs. We also investigate their role in this section by designing three set-ups, \textit{random string inputs}, \textit{OOD inputs}, and \textit{random question inputs}. The original input texts are replaced by random ASCII strings, OOD sentences, and random questions from the support datasets, respectively. The OOD sentences are randomly chosen from CC-News~\cite{ccnews}, a dataset containing news articles from news sites worldwide. Fig.~\ref{fig:understand-input} shows the results from these different question demonstration settings. Questions consisting of random strings do not have as much decrease in performance as OOD questions and random questions. OOD and random questions have a negative impact on ICL performance especially when the number of shots increases. 

The format of the context examples is the use of input-label pairing. Although there are many aspects of the format that can be changed, we make minimal modifications following the setting in~\cite{min-etal-2022-rethinking}. Specifically, three different formats are designed for VQA and GQA tasks. The labels are removed in setting \textit{no labels}; questions are removed in \textit{only labels}; and both questions and labels are removed in \textit{no questions and no labels}. Performances under these three settings are in Fig.~\ref{fig:understand-format}. In comparison to the ground-truth scenario, \ie, demonstrations include the whole instructions, omitting labels directly leads to $0$ performances, whereas only excluding the questions remains a major part of the performances, which again indicates the importance of correct label space.



% \subsection{Format of input-label pairing}
% \label{sec:understanding:format_input_label_pairing}


% Conclusion 

% \TODO{Exps on different Ordering }



==> sections/old-4-analysis.tex <==
% Jindong
% Improvement: target space-aware instructions for improving ICL.

\section{Discussion}
% merged to Section 6.3
%% language backbone 
%% visual encoder 
